Random Spreading for Unsourced MAC with Power Diversity

We propose an improvement of the random spreading approach with polar codes for unsourced multiple access. Each user encodes its message by a polar code, and the coded bits are then spread using a random spreading sequence. The proposed approach divides the active users into different groups, and employs different power levels for each group in such a way that the average power constraint is satisfied. We formulate and solve an optimization problem to determine the number of groups, and the number of users and power level of each group. Extensive simulations show that the proposed approach outperforms the existing methods, especially when the number of active users is large.

==> Makefile <==
# $Id: Makefile,v 1.7 2003/06/22 09:23:35 m Rel $

NAME=soul
ARCHNAME=$(NAME).tar.gz
ARCHIVE=$(NAME).dtx Makefile $(NAME).txt $(NAME).ins
MAKEIDXOPT=
DVIPSOPT=#-Pcmz -Pamz
DEP=$(NAME).sty

all: $(NAME).sty $(NAME).ps

print: $(NAME).ps
	psbook $(NAME).ps|psnup -2|psselect -e|lpr
	@ echo -n revert paper stack and hit return
	@ read key
	psbook $(NAME).ps|psnup -2|psselect -o -r|lpr

ps: $(NAME).ps

%.ps: %.dvi
	dvips $(DVIPSOPT) $< -o $@

hyper: $(NAME).dtx $(NAME).sty
	pdflatex "\relax\let\makehyperref\active\input $(NAME).dtx"

$(NAME).pdf: $(NAME).dtx $(NAME).sty
	pdflatex $(NAME).dtx

archive:
	@ tar -czf $(ARCHNAME) $(ARCHIVE)
	@ echo $(ARCHNAME)

clean: 
	rm -f $(NAME).{log,toc,lot,lof,idx,ilg,ind,aux,blg,bbl,dvi,ins,out}

distclean: clean
	rm -f $(NAME).{ps,sty,pdf} $(ARCHNAME)


REFWARN = 'Rerun to get cross-references'
LATEXMAX = 5

%.dvi: %.dtx $(DEP)
	latex $< ; true
	RUNS=$(LATEXMAX); \
	while [ $$RUNS -gt 0 ] ; do \
		if grep $(REFWARN) $*.log > /dev/null; \
		then latex $< ; else break; fi; \
		RUNS=`expr $$RUNS - 1`; \
	done

$(NAME).sty: $(NAME).ins soul.dtx
	tex $(NAME).ins

$(NAME).ins:
	latex $(NAME).dtx


